Discovering Object Masks with Transformers for Unsupervised Semantic Segmentation

The task of unsupervised semantic segmentation aims to cluster pixels into semantically meaningful groups. Specifically, pixels assigned to the same cluster should share high-level semantic properties like their object or part category. This paper presents MaskDistill: a novel framework for unsupervised semantic segmentation based on three key ideas. First, we advocate a data-driven strategy to generate object masks that serve as a pixel grouping prior for semantic segmentation. This approach omits handcrafted priors, which are often designed for specific scene compositions and limit the applicability of competing frameworks. Second, MaskDistill clusters the object masks to obtain pseudo-ground-truth for training an initial object segmentation model. Third, we leverage this model to filter out low-quality object masks. This strategy mitigates the noise in our pixel grouping prior and results in a clean collection of masks which we use to train a final segmentation model. By combining these components, we can considerably outperform previous works for unsupervised semantic segmentation on PASCAL (+11% mIoU) and COCO (+4% mask AP50). Interestingly, as opposed to existing approaches, our framework does not latch onto low-level image cues and is not limited to object-centric datasets. The code and models will be made available.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We refer to the introduction in Section~\ref{sec: introduction}.}
  \item Did you describe the limitations of your work?
    \answerYes{Section~\ref{sec: limitations} discusses the limitations of our approach. We also present two future directions.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We refer to the Broader Impact paragraph in Section~\ref{sec: broader_impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide all necessary information in the main paper and suppl. materials to reproduce the results (see experimental setup in Section~\ref{sec: experimental_setup}). Code and pre-trained models will be released upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We have included the main training details in the paper (see Section~\ref{sec: experimental_setup}). We mention additional details (\eg, augmentations) in the suppl. materials (see Section A)}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{All results are averaged of 5 runs, which is inline with prior work~\cite{he2019momentum,van2021unsupervised}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We refer to the implementation details in the suppl. materials (see Section A).}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
\answerYes{We cite all used assets. This includes the code, datasets and models.}
  \item Did you mention the license of the assets?
    \answerYes{All assets are publicly available and free to use for research purposes. We refer to the suppl. materials for more details.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    %\answerYes{We provide the pseudocode of our algorithm in the suppl. materials. Code and models will be made publicly available under an academic license upon acceptance.}
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

